Interface-resolved simulation of the evaporation and combustion of a fuel droplet suspended in normal gravity

An interface-resolved simulation of the combustion of a fuel droplet suspended in normal gravity is presented in this work, followed by an extensive analysis on the physical aspects involved. The modeling is based on DropletSMOKE++, a multiphase solver developed for the modeling of droplet vaporization and combustion in convective conditions. A wide range of phenomena can be described by the model, including the interface advection, the phase-change, the combustion chemistry, non-ideal thermodynamics and multicomponent mixtures. To our knowledge, this is the most detailed simulation performed on this configuration, providing a useful theoretical and numerical support for the experimental activity on this field. A recent experimental work is used as a reference, in which a methanol droplet is suspended on a quartz fiber and ignited at different oxygen concentrations. The numerical analysis offers a detailed insight into the physics of the problem and a satisfactory agreement with the experiments in terms of diameter decay, radial temperature profiles and sensitivity to the oxygen concentration. The vaporization rate is affected by the thermal conduction from the fiber, due to the high temperatures involved. Moreover, the fiber perturbs the flame itself, providing quenching at its surface. The combustion physics is compared to the one predicted at zero-gravity, evidencing a lower standoff-ratio, a higher flame temperature and an intense internal circulation. The distribution of the species around the droplet shows (i) a local accumulation of intermediate oxidation products at the fiber surface and (ii) water absorption in the liquid phase, affecting the vaporization rate.

==> backup.tex <==
\subsection{Data generation}
\todo[inline]{Actually I am testing a database based on laminar counterflow flames and it seems to work much better than PaSR. Thus this section will be rewritten}
The generation of sample data is of crucial importance for successfully applied the SOM procedure. In the present work the samples were generated by means of Partially Stirred Reactor (PaSR) calculations, similarly to what already done by Blasco et al. [REF] and by Liang et al. [REF]. The PaSR is often used as a reference configuration for developing, testing and validating reduced kinetic mechanisms. The PaSR model here adopted is described in detail by Chen [REF]. In this section only the most relevant features are presented. The reactor is represented by a large number $n_p$ of particles (Monte Carlo or stochastic particles). The PaSR is continuously fed by a specified number of inflow streams with prescribed composition and mass flow rate.
The mixing process in the PaSR is characterized by the mixing time $\tau_{mix}$, which is prescribed as an input parameter, together with the mean reactor residence time $\tau_{res}$. When the mixing time approaches zero, the mixing process becomes fast enough that the properties inside the PaSR are homogeneously mixed at the molecular level. In this limit, the PaSR becomes a Perfectly Stirred Reactor. On the contrary, in case of large mixing time, there is no mixing among the pockets of gas in the PaSR. Consequently, the PaSR consists of segregated reactive mixtures.
The chemical composition and the temperature of each particle evolve in time in small time steps $\Delta t$, in three sequential fractional steps: inflow/outflow, mixing and reaction.  In the inflow/outflow step, a number $n_{in}=n_p \Delta t / \tau_{res}$ of particles is randomly selected and their composition is replaced by composition of inflow streams. Similarly, in the mixing step, according to the Modified Coalescence Dispersion (MCD) model, $n_{mix}=C_{mix} n_p \Delta t / \tau_{mix}$ pairs of particles is chosen, where $C_{mix}$ is a model parameter, here assumed equal to $1/2$. For each pair, the composition and the enthalpy of both particles is put equal to the corresponding arithmetic average, in order to simulate the mixing. In the reaction fractional step, the thermo-chemical state of each particle evolves because of chemical reactions in isobaric, adiabatic conditions over the time step $\Delta t$. 
The simplicity of the PaSR model allows to carry out simulations with detailed chemistry without significant computing burden. From the general view of modeling reactive flows, PaSR can be viewed as a single grid cell embedded in a large computational scheme. Consequently, PaSR offers an ideal system for generating sample data which are sufficiently representative of multidimensional flames.

\subsection{Generation of sample data}
\todo[inline]{See previous comment}
The sample data were generated by means of PaSR simulations. The residence time was assumed equal to 10 ms, while five different mixing times were considered (from 0.5 to 5 ms). 500 stochastic particles were considered, whose initial composition was set to the thermodynamic equilibrium composition. The PaSR was run for 10 residence times. A sample composition database containing $n_D=50,000$ distinct compositions was assembled by sampling the particles in the reactor over the entire duration of the simulations. Figure \ref{fig:pasr_averages} shows the evolution of average (ensemble) temperature for the five different simulations here adopted. It is evident that the range of chosen mixing times is sufficiently large to cover a wide area of composition space, from thermodynamic equilibrium to extinction. The Supplementary Materials provides additional results about the PaSR simulations. 


In order to have a proper partitioning, it is important to choose correctly the input variables. In this work, instead of using directly the $n_s+1$ thermo-chemical variables (species and temperature), a proper number of principal components is adopted. In particular, the original thermo-chemical variables $\bf{\psi}$ are standardized, in order to have a new set of variables $\bf{\phi}$ centered (i.e. with mean equal to 0) and scaled (i.e. with standard deviation equal to 1):
\begin{equation}
\phi_{i,j}=\frac{\psi_{i,j}-\mu_i}{\sigma_i} \quad j=1,...,n
\end{equation}
where $\mu_i$ and $\sigma_i$ are the mean and the standard deviation of original variable $i$ and $n$ is the total number of thermo-chemical states (samples).
The principal components of rescaled variables $\bf{\phi}$ are then calculated. The first $n_{pca}$ components are retained and used as input data for the SOM. In particular, $n_{pca}$ is chosen as the minimum number of components explaining $99\%$ of total variance. 
Each principal component is a linear combination of the original variables and all the principal components are orthogonal to each other, so there is no redundant information. Thus, this allows to reduce the number of significant variables for the SOM. This definition of input variables has some important advantages: i) it is cheap to evaluate (which is essential for fast classification during the CFD simulation); ii) most of the compositional variance is retained, which is expected to result in a good selectivity when classifying the compositions.


By comparing the size of the final mechanism with the average size of individual mechanisms, it is also possible to have a simple estimation of the quality of the partitioning procedure (see Section 3).

In particular, the SOM architecture is like that of a competitive network, except no bias is used. The competitive transfer function produces 1 for the output element corresponding to the winning neuron (i.e. the cluster). All other output elements are 0. 

The values of its components are in general a good indication of how the multidimensional input space is classified (or projected) on the 2D SOM. 

Previous simulations demonstrated that such a mesh was sufficiently fine for correctly describing the unsteady behavior of the flame [REF]. 

About 85\% of total CPU time is spent for solving the chemical step, 10\% for the transport step, and the remaining 5\% for calculating the transport properties and for carrying out additional tasks. Since the adaptive chemistry algorithms acts on the chemical sub-step only, the maximum theoretical overall speed-up factor we can expect is $~6$.



\section{Introduction}
Detailed kinetics is today recognized as a key element for predictive simulation of laminar and turbulent flames aimed at more effective design of combustion devices (such as internal combustion engines and gas turbines). However, the coupling of Computational Fluid Dynamics (CFD) and detailed chemistry is computationally demanding, mainly because of the large number of species and the wide range of chemical times typically involved in detailed chemistry \cite{Lu2009192}. During the last years, several techniques have been proposed for reducing the computational cost associated with the adoption of detailed kinetic mechanisms. One of the most popular is the automatic reduction technique to produce skeletal mechanisms, with a reduced number of species and reactions \cite{Lu20051333}. However, even if reduced mechanisms are adopted, the computational cost is not always feasible, especially in the context of LES and DNS, where the time spent for chemistry calculations can take most of the total CPU time. 
\newline
If inhomogeneous reactive flows are solved by numerical schemes based on the operator-splitting strategy \cite{Ren20088165}, additional and more effective techniques can be considered for reducing the computational cost of detailed chemistry. In operator-splitting methods, most of the CPU time is spent in the chemical step, which corresponds to the solution of $N$ (with $N$ being the total number of computational cells) independent, stiff and non linear systems of ordinary differential equations (ODEs): 
\begin{equation}
\frac{d\boldsymbol{\psi}}{dt}=\boldsymbol{S}(\boldsymbol{\psi})
\end{equation}
where $\boldsymbol{\psi}$ is the thermo-chemical state vector (composition+temperature) in a single cell and $\boldsymbol{S}(\boldsymbol{\psi})$ is the corresponding rate of change due to chemical reactions. Since the ODE systems above are independent, techniques based on adaptive chemistry are very effective and easy to implement. They are based on the observation that in any small range of temperature and compositions many species have negligible concentrations and only a limited number of them is chemically active. In other words, this means that the effective kinetic mechanism locally (in the thermo-chemical space) needed for describing the chemical evolution may require fewer species and reactions than the complete mechanism applicable over the whole thermo-chemical space. In principle, the maximum  level of adaptivity, which means the maximum level of reduction, can be achieved through the Dynamic Adaptive Chemistry (DAC) approach \cite{Liang2009527,Contino20113057}: at each time step of the simulation the local thermo-chemical state is analyzed, the important reactions and species are recognized and only the corresponding equations governing their evolution are solved, while the unimportant species are considered as inert species. This means that the evolution in each cell is described through a local kinetic mechanism. Unfortunately, the computational cost needed for selecting the important species and reactions is often very large (especially if high levels of reduction are required). 
\newline 
In order to reduce the additional cost of adaptive reduction, it is possible to build in a pre-processing phase a library of reduced mechanisms covering the chemical regimes which are expected in the flame of interest, similarly to what already proposed by Schwer et al. \cite{Schwer2003451} and Banerjee and Ierapetritou \cite{Banerjee2006619}. A first problem is represented by the fact that the accessed region is not known \textit{a priori}. Partially Stirred Reactors (PaSR) \cite{Liang2015} or unsteady laminar flamelets \cite{Franke2017245} are typically adopted for covering the accessed region. A second issue to be faced is the proper pre-partitioning of the accessed region in a reasonably small number of \textit{clusters}, for which a library of reduced kinetic mechanism can be generated. The difficulty is in partitioning the composition space in clusters before the derivation of reduced kinetic mechanisms, ensuring that each individual cluster is sufficiently homogeneous from the reactive point of view, i.e. that a single reduced kinetic mechanism is able to correctly describe all the composition samples belonging to it \cite{Liang2015}. In particular, Self Organizing Maps (SOM) have been successfully adopted for partitioning the composition space by Blasco et al. \cite{Blasco200061} and more recently by Franke et al. \cite{Franke2017245}, showing important advantages in terms of computational efficiencies and storage requirements.
\newline
In this paper we present and apply a new methodology for including detailed chemistry in multidimensional CFD simulations based on the coupling between Self Organizing Maps (SOM) \cite{Kohonen1995} and mechanism reduction via DRGEP (Directed Relation Graph with Error Propagation) \cite{Pepiot-Desjardins20081089}. Rather than performing \textit{on the fly} chemical reduction, an analysis of the composition space likely to be accessed during the combustion simulation is carried out in a pre-processing phase by means of Partially Stirred Reactor (PaSR) and steady state laminar counter flow diffusion flame (CFDF) simulations. Then, the generated composition space is pre-partitioned in a number of clusters via SOM and for each cluster a reduced kinetic mechanism is generated. The CFD simulation is carried out by transporting the whole set of chemical species included in the detailed mechanism. However, before carrying out the chemical step, each cell is classified using the same SOM adopted for pre-partitioning the composition space, in order to identify the cluster to which the cell belongs (and therefore select the corresponding reduced mechanism). Since the cluster identification through the SOM is very fast and the mechanism reduction is entirely carried out in the pre-processing step, the run-time overhead associated to the adaptive chemistry strategy is kept to a minimum.
This article is structured as follows. In Section 2 details about the methodology are reported. In Section 3 we present an example of application to non-premixed combustion of methane in air. In particular, after presenting and discussing the pre-partitioning results (by analyzing different SOM clusterings), the simulation of a 2D forced, time-varying, laminar diffusion flame is presented and analyzed. Conclusions are provided in Section 4.

\begin{table}[tbp]
\centering
\caption{Average errors between complete and adaptive chemistry simulations for temperature and selected mass fractions }
\label{tab:errors}
\begin{tabular}{lllll}
$n_{som}$  & $\epsilon$ & $E_{T}$ & $E_{OH}$ & $E_{CO}$  \\
%som   eps      ET        EOH         ECO         
 25  & 0.005  & 1.11e-4   & 1.44e-4   & 1.03e-3     \\
 25  & 0.010  & 1.15e-4   & 1.54e-4   & 1.57e-3     \\
 25  & 0.020  & 1.16e-4   & 1.61e-4   & 1.65e-3     \\
 49  & 0.010  & 1.05e-4   & 1.40e-4   & 0.96e-3     \\
 81  & 0.010  & 1.04e-4   & 1.37e-4   & 0.93e-3     \\
\end{tabular}
\begin{tablenotes}\footnotesize
\item[*] Only cells with $T>300 K$ were accounted for in the averaging process. A mass fraction threshold of $10^{-6}$ was considered for $E_{OH}$ and $E_{CO}$.
\end{tablenotes}
\end{table}
